AUTOLEX: An Automatic Framework for Linguistic Exploration

Each language has its own complex systems of word, phrase, and sentence construction, the guiding principles of which are often summarized in grammar descriptions for the consumption of linguists or language learners. However, manual creation of such descriptions is a fraught process, as creating descriptions which describe the language in "its own terms" without bias or error requires both a deep understanding of the language at hand and linguistics as a whole. We propose an automatic framework AutoLEX that aims to ease linguists' discovery and extraction of concise descriptions of linguistic phenomena. Specifically, we apply this framework to extract descriptions for three phenomena: morphological agreement, case marking, and word order, across several languages. We evaluate the descriptions with the help of language experts and propose a method for automated evaluation when human evaluation is infeasible.

==> ExperimentalSetup.tex <==

\section{Experimental Setup}
\label{sec:setup}
\an{The first sentence is quite repetitive, could summarize}
To answer \emph{how well our framework can discover the conditions  which govern the different linguistic phenomena that apply to the language in general}, we train models to answer questions about word order, morphological agreement, and case marking for several languages which have expert-annotated syntactic analysis readily available. We refer to these as gold-standard experiments (Section \S\ref{sec:goldexptauto}).
Next, we manually verify these extracted rules (Section \S\ref{sec:goldexptmanual}).
Finally, we conduct a case study for an endangered language and evaluate \emph{how effective our framework is   when we don't have access to the expert syntactic analysis}  (Section \S\ref{sec:lowexpt}).


%\paragraph{Data}
\paragraph{Data and Model}
For the gold-standard experiments, we use the Syntactic Universal Dependencies (SUD) \cite{gerdes-etal-2019-improving} treebanks which are based on the Universal Dependencies (UD) \cite{nivre2016universal,nivre2018universal} project, the difference being that SUD treebanks allow function words to be syntactice heads (as opposed to UD's preference for content words), which is more conducive to our goal of learning grammar rules.  
These treebanks are publicly available for 71 languages with annotations for POS tags, lemmas, dependency parses and morphological analysis.
We use the same train, validation and test split as provided in the treebanks to create the training data to answer each linguistic question.
We use the \texttt{XGBoost} \cite{chen2016xgboost} library to learn the decision tree. Details on the model setup are discussed in Appendix \ref{sec:modelsetup}.
 
%, from which we then extract the human- and machine-readable rules.
% As described in Section \S\ref{sec:traindata}, we train a separate model for each linguistic question and language.
% We perform grid search over a set of hyperparameters and select the model which performs best on the validation set. We describe the details 


%\paragraph{Model}


==> images/greekexample.tex <==
\begin{figure*}[t]
\centering
\label{sentpart-1}%
\begin{dependency}[edge slant=5pt,label theme = simple, edge theme = iron]
  \begin{deptext}[column sep=1em]
    \textgreek{Οι} \& \textgreek{διατάξεις} \& \textgreek{αυτές} \& \textgreek{αντιστοιχούν} \& \textgreek{σ} \& \textgreek{τα} \&\textgreek{πρότυ} \\
    \small{the.DET} \& \underline{\small{provision.N.Nom}} \& \small{these.PRON.Nom} \& \small{correspond.V} \& \small{ADP} \& \small{DET} \& \small{standards.N.Acc} \&   \\
  \end{deptext}
  \deproot[edge height=3em]{4}{ROOT}
  \depedge[edge height=1em]{2}{3}{DET}
  \depedge[edge height=2.5em]{4}{2}{SUBJ}
  \depedge[edge height=1em]{5}{4}{UDEP}
  %\depedge[edge height=1.9cm]{7}{2}{TMOD}
  %\depedge{2}{3}{aux}
 \depedge[edge height=1em]{7}{5}{OBJ}
  %\depedge{5}{4}{det}
  %\depedge{3}{6}{punct}
%   \depedge{7}{9}{ADVMOD}
%   \depedge[edge start x offset=-4pt]{9}{8}{ADVMOD}
\end{dependency}
\caption{Examples of case variation in Greek nouns. For the above sentence -- ``these \underline{provisions} correspond to the standards'', the underlined \underline{noun} takes the nominative case because it is the subject of the main verb. The pronoun also takes the nominative case because its the determiner of the noun which is the subject. A noun takes the accusative case when it is the object.   \aditi{check the example with Antonios}.}%
\label{fig:casemarking}%
\end{figure*}



==> images/marathiexample.tex <==
\begin{figure}[t]
    \centering
    \small
    \begin{tabular}{@{}lllll}
        \multirow{1}{*}{A.1} & Meera &  & pustake & watch-te \\
         & \small{Meera.3P.SG} &  & \small book.N.PL & \small read-IPFV \\
         & \multicolumn{4}{l}{`Meera reads books.'}\\
         \midrule
        \multirow{1}{*}{A.2} & Meera & \textcolor{blue}{ne} & pustake & watch-li \\
         & \small{Meera.3P.SG} & \small ERG & \small book.N.PL & \small read-PFV\\
         & \multicolumn{4}{l}{`Meera read books.'}\\
         \midrule 
        \multirow{1}{*}{A.3} & me & \textcolor{red}{*ne} & pustake & watch-li \\
         & \small{I.1P.SG} & \small ERG & \small book.N.PL & \small read-PFV \\
          & \multicolumn{4}{l}{`I read books.'}\\
         \midrule
         \multirow{1}{*}{A.4} & courta & \textcolor{blue}{ne} & faisla & dila \\
         & \small{court.SG} & ERG & \small decision.N & \small give-PFV \\
         & \multicolumn{4}{l}{`Court gave the decision.'}\\
         \midrule 
         
    \end{tabular}
    
    \caption{Ergative case marking in Marathi. A.1 shows for verbs in imperfective aspect, 3rd person singluar subjects do not take the ergative case marker (\textbf{ne}), whereas they do so for  perfective verbs, as in example A.2. Example A.3 shows that 1st person singular subjects  do not take the ergative marking for perfective verbs. 
    Apart from syntactic features, animacy in example A.4 shows that even inanimate nouns as `court' can take the ergative case when used as a volitional entity.
    }
    \label{fig:marthimarkingexample}
    \vspace{-1em}
\end{figure}



==> images/sentenceTypeExample.tex <==
\begin{figure}[t]
\centering
\subfigure[(Most) Declarative sentences show subject-verb-object. ]{%
\label{sentpart-1}%
\begin{dependency}[edge slant=5pt,label theme = simple, edge theme = iron]
  \begin{deptext}[column sep=1em]
    Peter \& is \& \underline{eating} \& the \& fruit \& . \\
  \end{deptext}
  \deproot[edge height=1.5em]{3}{ROOT}
  \depedge[edge height=1em]{3}{1}{SUBJ}
  %\depedge[edge height=1.9cm]{7}{2}{TMOD}
  %\depedge{2}{3}{aux}
  \depedge[edge height=1em]{3}{5}{OBJ}
  %\depedge{5}{4}{det}
  %\depedge{3}{6}{punct}
%   \depedge{7}{9}{ADVMOD}
%   \depedge[edge start x offset=-4pt]{9}{8}{ADVMOD}
\end{dependency}}
%~
\subfigure[(Some) Interrogative sentences show object-subject-verb.]{%
\label{sentpart-2}%
\begin{dependency}[edge slant=5pt,label theme = simple, edge theme = iron]
  \begin{deptext}[column sep=1em]
    What \& is \& Peter \& \underline{eating} \& ? \\
  \end{deptext}
  \deproot[edge height=1.5em]{4}{ROOT}
  \depedge[edge height=1.2em]{4}{1}{OBJ}
  \depedge[edge height=0.4em]{4}{3}{SUBJ}
\end{dependency}}
\caption{Example of word order variations in English.}%
\label{fig:wordorder}%
\end{figure}

==> images/spanishexample.tex <==
% several cities were decorated.
%varias ciudades fueron decoradas.
% the new professor is loud.
%el nuevo profesor es ruidoso.
% Four books were bought.
%Se compraron cuatro libros.
% the big house was painted. 
%la casa grande fue pintada.

% \begin{figure}[t]
% %\centering
% \subfigure[Several cities were decorated.]{
% \label{fig:spapart1}
% \begin{dependency}[edge slant=5pt,label theme = simple, edge theme = iron]
%   \begin{deptext}[column sep=1em]
%     \small{\textbf{varias}} \&\small{\underline{ciudades}} \& \small{fueron} \& \small{decoradas} \\
%     \small{varios.ADJ} \& \small{ciudad.N} \& \small{ser.AUX} \& \small{decorado.ADJ}  \\ 
%     %\small{NumType=Ord} \& \small{FEM.PL} \&  \& \& \small{FEM.SG} \&  \small{SG}   \\
%   \end{deptext}
%   \depedge[edge height=1em]{2}{1}{MOD}
% \end{dependency}
% }
% %~
% \subfigure[The new professor is loud]{
% \label{fig:spapart2}
% \begin{dependency}[edge slant=5pt,label theme = simple, edge theme = iron]
%   \begin{deptext}[column sep=1em]
%   \small{el} \& \small{\textbf{nuevo}} \& \small{\underline{profesor}} \& \small{es}  \& \small{ruidoso} \\
%     \small{el.DET} \& \small{nuevo.ADJ} \& \small{profesor.N} \& \small{es.V} \& \small{ruidoso.ADJ}  \\ 
%   \end{deptext}
%   \depedge[edge height=1em]{3}{2}{MOD}
% \end{dependency}
% }
% %~
% \subfigure[Four books were bought]{
% \label{fig:spapart3}
% \begin{dependency}[edge slant=5pt,label theme = simple, edge theme = iron]
%   \begin{deptext}[column sep=1em]
%     \small{Se} \& \small{compraron} \& \small{\textbf{cuatro}} \& \small{\underline{libros}} \\
%     \small{se.PRON} \& \small{comprar.V} \& \small{cuatro.ADJ.Ord} \& \small{libro.N}  \\ 
%   \end{deptext}
%   \depedge[edge height=1em]{4}{3}{MOD}
% \end{dependency}
% }
% %~
% \subfigure[You have a big house]{
% \label{fig:spapart4}
% \begin{dependency}[edge slant=5pt,label theme = simple, edge theme = iron]
%   \begin{deptext}[column sep=1em]
%     \small{Tienes} \& \small{una} \& \small{\underline{casa}} \& \small{\textbf{grande}} \\
%     \small{tener.AUX} \& \small{uno.DET} \& \small{casa.N.} \& \small{grande.ADJ}  \\ 
%   \end{deptext}
%   \depedge[edge height=1em]{3}{4}{MOD}
% \end{dependency}
% }
% \caption{Examples of adjective-noun word order variations in Spanish.
% Usually \textbf{adjectives} come after \underline{nouns}. There are exceptions where  adjectives can come before nouns such as ordinals,  adjectives denoting quantity, or specific adjectives such as \textbf{nuevo, grande} which can come both before or after. \gn{Proposal here: Could you reduce the number of sentences to only one sentence, and then have the features extracted for each word listed beneath each word? Each category of features (syntactic, lexical, semantic) could be surrounded by a different-colored box.} }%
% \label{fig:spanishwordorderexample}%
% \end{figure}


\begin{figure}[t]
    \centering
    \includegraphics[width=\columnwidth]{images/Feature.pdf}
    \caption{Features extracted for training the adjective-noun word order model in Spanish. The sentence translates to ``\textbf{Four} \underline{books} were bought''.} 
    % \gn{Are the ``lemma-is-cuatro'' and ``lemma-is-libro'' actually ``dep-lemma-is-quatro'' and ``head-lemma-is-libro''? I think you make a distinction here, right?}\aditi{yeah, thats correct, I did make a distinction, I have fixed it in the figure also, thanks!} }
    \label{fig:spanishwordorderexample}
\end{figure}

==> problemformulation.tex <==
\section{Problem Formulation}
% \gn{I feel that this is a bit redundant with the intro}
We then determine the set of $k$ features   which may be useful in describing the phenomena ($\mathbf{x_i}=x_i^0, x_i^1, \cdots, x_i^k$) and extract these features from text of the language of interest, often aided by local syntactic analysis such as a dependency parsing or morphological analysis.  
Once we define the input and output to the classification task, we fit an interpretable model $\Theta_p$ over the extracted data, from which we then extract the desired rule-sets $R_p$. 
% As mentioned earlier, we explore three linguistic phenomena though this general question. Specifically, here the research questions we ask:
% \begin{itemize}
%   \item \textbf{Case Marking}: When does a particular class of words (e..g nouns) take one case (e.g. nominative) over the other? (Section \S\ref{sec:marking})
  
%   \item \textbf{Word Order}: When is one word order (e.g. subject-verb) predominant over the other? (Section \S\ref{sec:wordorder})
  
%   \item \textbf{Agreement}: When do syntactic heads show morphological agreement (e.g. subject-verb gender agreement) with their dependents? (Section \S\ref{sec:agreement})
% \end{itemize} 
